Recycling Scraps: Improving Private Learning by Leveraging Intermediate Checkpoints

In this work, we focus on improving the accuracy-variance trade-off for state-of-the-art differentially private machine learning (DP ML) methods. First, we design a general framework that uses aggregates of intermediate checkpoints \emph{during training} to increase the accuracy of DP ML techniques. Specifically, we demonstrate that training over aggregates can provide significant gains in prediction accuracy over the existing state-of-the-art for StackOverflow, CIFAR10 and CIFAR100 datasets. For instance, we improve the state-of-the-art DP StackOverflow accuracies to 22.74\% (+2.06\% relative) for $\epsilon=8.2$, and 23.90\% (+2.09\%) for $\epsilon=18.9$. Furthermore, these gains magnify in settings with periodically varying training data distributions. We also demonstrate that our methods achieve relative improvements of 0.54\% and 62.6\% in terms of utility and variance, on a proprietary, production-grade pCVR task. Lastly, we initiate an exploration into estimating the uncertainty (variance) that DP noise adds in the predictions of DP ML models. We prove that, under standard assumptions on the loss function, the sample variance from last few checkpoints provides a good approximation of the variance of the final model of a DP run. Empirically, we show that the last few checkpoints can provide a reasonable lower bound for the variance of a converged DP model. Crucially, all the methods proposed in this paper operate on \emph{a single training run} of the DP ML technique, thus incurring no additional privacy cost.

==> abstract.tex <==
\begin{abstract}
In this work, we focus on improving the  accuracy-variance  trade-off for state-of-the-art (SOTA) differentially private machine learning (DP ML) methods. First, we design a general framework that uses aggregates of intermediate checkpoints \emph{during training} to increase the accuracy of DP ML techniques. Specifically, we demonstrate that training over aggregates can  provide significant gains in prediction accuracy over the existing SOTA for StackOverflow and CIFAR10 datasets, and that these gains get magnified in settings with periodically varying training data distributions. For instance, we improve  SOTA DP StackOverflow accuracies to 22.74\% (+2.06\% relative) for $\epsilon=8.2$, and 23.90\%  (+2.09\%) for $\epsilon=18.9$. Lastly, we initiate an exploration into estimating the uncertainty (variance) that DP noise adds in the predictions of DP ML models. We prove that, under standard assumptions on the loss function, the sample variance from last few checkpoints provides a good approximation of the variance of the final model of a DP run. Empirically, we show that the last few checkpoints can provide a reasonable lower bound for the variance of a converged DP model. Crucially, all the methods proposed in this paper operate on \emph{a single training run} of the DP ML technique, thus incurring no additional privacy cost.
\end{abstract}

==> app-checkpoint.tex <==
\section{Proof of Theorem~\ref{thm:tail}}
\label{app:tail}

\begin{proof}
We adapt the proof from Theorems 2 and 4  of~\cite{shamir2013stochastic}. If we choose $T = \lceil n \rho\rceil$ and set $\eta_t$ appropriately, the proof of Theorem 2 \citep{shamir2013stochastic} implies the following for $\theta^{\sf UTA}_T$:
$$\mathbb{E}\left[\calL\left(\theta^{\sf UTA}_T;D\right)\right]-\min\limits_{\theta\in\calC}\calL(\theta;D) = O\left(\frac{L \ltwo{\calC} \sqrt{p}}{n \rho} \log\left(\frac{1}{\alpha}\right)\right).$$

Setting $\alpha = \Theta(1)$ gives the theorem's first part, and $\alpha T = 1$, i.e., $1/\alpha = T = \lceil n \rho \rceil$ gives the second.
The third follows from modifying Theorem 4 of \cite{shamir2013stochastic} for the convex case (see the end of Section 4 of \cite{shamir2013stochastic} for details).
\end{proof}


==> preliminaries.tex <==





==> uta.tex <==
\section{Improving DP-ML accuracy by Uniform Tail Averaging of DP training checkpoints}\label{acc}
In this section, we first discuss DP preliminaries. Then we describe our first checkpoints aggregation proposal: \emph{uniform tail averaging (UTA)} and give theoretical guarantees on improved privacy-utility trade-offs due to UTA. Then, we discuss five intuitive checkpoints aggregation methods in section~\ref{acc:additional_aggs}. Next, we present experiments that demonstrate the significantly improved privacy-utility trade-offs due to our checkpoints aggregation methods in a user-level DP Federated Learning (FL) setting. Finally, we present experiments with sample-level DP. 

\input{preliminaries}
\vspace*{-.25em}
\subsection{Uniform tail averaging of DP checkpoints}\label{acc:uta}

Our first proposal uniform tail averaging (UTA) is a checkpoints aggregation method of type \emph{parameters aggregation}; parameters aggregation methods compute a function of the parameters of intermediate checkpoints from a DP run and use the resulting aggregate parameters for inference. More specifically, for step $t$ of DP training, UTA computes the \emph{parameter-wise} mean of the past $k$ checkpoints, i.e., checkpoints from steps $[t-(k-1), t]$. We formalize this as: $\theta^{t,k}_\text{uta} = \frac{1}{k} \sum^{t}_{i=t-(k-1)} \theta^{i}\label{param_upa}$.

Note that UTA (and other checkpoints aggregation methods in Section~\ref{acc:additional_aggs}) \emph{post-process} the already DP checkpoints, and hence, do not incur any additional privacy cost. Furthermore, UTA is general method that is applicable to any training algorithm that computes intermediate checkpoints.

\subsubsection{Improved excess risk via UTA}
\label{acc:theory}

In this section, we formally show that checkpoint aggregations like uniform tail averaging provably improves the privacy/utility trade-offs, compared to that of the last checkpoint of DP-SGD. To formalize the problem, we define the following notation: Consider a data set $D=\{d_1,\ldots,d_n\}$ and a loss function $\calL(\theta;D)=\frac{1}{n}\sum\limits_{i=1}^n\ell(\theta;d_i)$, where each of the loss function $\ell$ is convex and $L$-Lipschitz in the first parameter, and $\theta\in\calC$ with $\calC\subseteq\mathbb{R}^p$ being a convex constraint set. 
We analyze the following variant of DP-SGD, which is guaranteed to be $\rho$-zCDP\footnote{Using~\cite{bun2016concentrated}, it is easy to convert the privacy guarantee to an $(\epsilon,\delta)$-DP guarantee.}.

\begin{enumerate}
    \item $\theta_0\leftarrow \mathbf{0}^p$.\vspace{-0.1cm}
    \item For $t\in[T]$, $\theta_{t+1}\leftarrow\Pi_{\calC}\left(\theta_t-\eta_t\left(\nabla\calL(\theta_t;D)+b_t\right)\right)$, where $b_t\sim\calN\left(0,\frac{L^2T}{2n\rho}\mathbb{I}_{p\times p}\right)$ and $\Pi_\calC\left(\cdot\right)$ being the $\ell_2$-projection onto the set $\calC$.
\end{enumerate}
We will provide the utility guarantee for this algorithm by directly appealing to the result of~\cite{shamir2013stochastic}. For a given $\alpha\in (0,1)$, UTA corresponds to the average of the last $\alpha T$ models, i.e., 
$\privTa=\frac{1}{\alpha T}\sum\limits_{t=(1-\alpha)T+1}^T\theta_t.$
One can also consider~\emph{polynomial-decay averaging} (PDA) with parameter $\gamma \geq 0$, defined as follows:
$\privTpoly[t]=\left(1-\frac{\gamma+1}{t+\gamma}\right)\privTpoly[t-1]+\frac{\gamma+1}{t+\gamma}\cdot\theta_t.$

For $\gamma = 0$, PDA matches UTA over all iterates. As $\gamma$ increases, PDA places more weight on later iterates; in particular, if $\gamma = cT$, the averaging scheme is very similar to EMA (Section~\ref{acc:additional_aggs}), since as $t \rightarrow T$ the decay parameter $\frac{\gamma+1}{t+\gamma}$ approaches a constant $\frac{c}{c+1}$. In that sense, PDA can be viewed as a method interpolating between UTA and EMA.
\begin{thm}[Adapted from Theorems 2 and 4 of~\cite{shamir2013stochastic}]
Consider the DP-SGD algorithm above, and the associated parameters. Then there exists choice of learning rate $\eta_t$ and the number of time steps $T$ s.t. the following are true for $\alpha=\Theta(1)$:

{\small
$\mathbb{E}\left[\calL\left(\privTa;D\right)\right]-\min\limits_{\theta\in\calC}\calL(\theta;D)=\calO\left(\frac{L\ltwo{\calC}\sqrt{p}}{n\rho}\right)$, 
and
$\mathbb{E}\left[\calL(\theta_T;D)\right]-\min\limits_{\theta\in\calC}\calL(\theta;D)=\calO\left(\frac{L\ltwo{\calC}\sqrt{p}\log(n)}{n\rho}\right).$}

Furthermore, for $\gamma=\Theta(1)$, we have,
$\mathbb{E}\left[\calL\left(\privTpoly[T];D\right)\right]-\min\limits_{\theta\in\calC}\calL(\theta;D)=\calO\left(\frac{L\ltwo{\calC}\sqrt{p}}{n\rho}\right).$
\label{thm:tail}
\end{thm}
\begin{proof}
If we choose $T = \lceil n \rho\rceil$ and set $\eta_t$ appropriately, the proof of Theorem 2 \citep{shamir2013stochastic} implies the following for $\privTa$:
$\mathbb{E}\left[\calL\left(\privTa;D\right)\right]-\min\limits_{\theta\in\calC}\calL(\theta;D) = O\left(\frac{L \ltwo{\calC} \sqrt{p}}{n \rho} \log\left(\frac{1}{\alpha}\right)\right).$

Setting $\alpha = \Theta(1)$ gives the theorem's first part, and $\alpha T = 1$, i.e., $1/\alpha = T = \lceil n \rho \rceil$ gives the second.
The third follows from modifying Theorem 4 of \cite{shamir2013stochastic} for the convex case (see the end of Section 4 of \cite{shamir2013stochastic} for details).
\end{proof}
The excess empirical risk for $\theta_T$ is higher by factor of $\log(n)$ in comparison to $\privTa$ and $\privTpoly[T]$. 
{For the step size selections typically used in practice (e.g., fixed or inverse polynomial step sizes), the last iterate will suffer from the extra $\log(n)$ factor, and we do not know how to avoid it. 
Furthermore, \cite{Harvey2019TightAF} showed that this is unavoidable in the non-private, high probability regime.\footnote{{\cite{Jain2021LastIterate} show that for carefully chosen step sizes, the logarithmic factor can be removed, and \cite{feldman2019private} extend this analysis to a  DP-SGD variant with varying batch sizes. Unlike those methods, averaging can be done as  post-processing of DP-SGD outputs, rather than a modification of the algorithm.}}}


\subsection{Additional checkpoints aggregation methods}\label{acc:additional_aggs}
Next, we discuss five additional intuitive checkpoints aggregation methods that we empirically evaluate in this work.

\mypar{UTA+} Note that, at step $t$, UTA uses the checkpoints aggregate $\theta^{t,k}_\text{uta}$ just for inference. However, in UTA+, instead of training over the most recent checkpoint $\theta^t$, we propose to train over the UTA aggregate, i.e., $\theta^{t,k}_\text{uta}$, of checkpoints. 

\mypar{Exponential moving average (EMA)} EMA has been previously used~\citep{tanle19, BrockDSS21} to improve the performance of ML models at inference time. 
Starting from the latest checkpoint of the run, EMA assigns exponentially decaying weights to each of the previous checkpoints; the weights are a function of the EMA \emph{coefficient $\beta_t$} at step $t$. During training, at each step $t$, EMA maintains a moving average $\theta^t_\text{ema}$ that is a weighted average of $\theta^{t-1}_\text{ema}$ and the $t^{th}$ checkpoint, $\theta^t$. This is formalized as follows: $\theta^t_\text{ema} = (1 - \beta_t) \cdot \theta^{t-1}_\text{ema} + \beta_t \cdot \theta^{t}$. Following \citep{tanle19, de2022unlocking}, we use a warm-up schedule for the EMA coefficient as: $\beta_t = \text{min}\left(\beta, ({1+t})/({10+t})\right)$.

\mypar{EMA+} Similar to UTA+, in EMA+, at step $t$, we propose to train on the EMA aggregate of checkpoints, i.e., $\theta^t_\text{ema}$, instead of training over the most recent checkpoint $\theta^t$.

\mypar{Output predictions averaging (OPA)} 
Recall that the aggregation methods discussed above are parameters aggregations.
We also propose two novel checkpoints \emph{outputs aggregation} methods, which compute a function of the outputs of the intermediate checkpoints, and use it for making predictions.
For a given test sample $\mathbf{x}$, OPA first computes prediction vectors $f_{\theta^{i}}(\mathbf{x})$ of the past $k$ checkpoints, i.e., checkpoints from steps $\in [t-(k-1), t]$, averages the prediction vectors, and computes argmax of the average vector as the final output label. We formalize OPA as $\hat{y}_\text{opa}(\mathbf{x}) = \text{argmax} \Big(\frac{1}{k} \sum^{t}_{i=t-(k-1)} f_{\theta^{i}}(\mathbf{x}) \Big)$.


\mypar{Output labels majority vote (OMV)}  For a given test sample $\mathbf{x}$, OMV computes output prediction vectors for $\mathbf{x}$ and the corresponding labels, i.e., $\text{argmax}\ f_{\theta^{i}}(\mathbf{x})$. Finally, it uses the majority label among the $k$ labels (breaking ties arbitrarily) as its final output label. We formalize OPA as $\hat{y}_\text{omv}(\mathbf{x}) =  \text{Majority} \big( \text{argmax}( f_{\theta^{i}}(\mathbf{x}) ) ^t_{i=t-(k-1)}\big)$.
